A Measure for Dialog Complexity and its Application in Streamlining Service Operations

Dialog is a natural modality for interaction between customers and businesses in the service industry. As customers call up the service provider, their interactions may be routine or extraordinary. We believe that these interactions, when seen as dialogs, can be analyzed to obtain a better understanding of customer needs and how to efficiently address them. We introduce the idea of a dialog complexity measure to characterize multi-party interactions, propose a general data-driven method to calculate it, use it to discover insights in public and enterprise dialog datasets, and demonstrate its beneficial usage in facilitating better handling of customer requests and evaluating service agents.

==> expt-insurance.tex <==
% -------------------------------------------------------------------
\subsubsection{Results with Insurance Data}

{\em Pavan to explain insurance tests}

% -------------------------------------------------------------------
